Don't Stop Me Now: Embedding Based Scheduling for LLMs

Efficient scheduling is crucial for interactive Large Language Model (LLM) applications, where low request completion time directly impacts user engagement. Size-based scheduling algorithms like Shortest Remaining Process Time (SRPT) aim to reduce average request completion time by leveraging known or estimated request sizes and allowing preemption by incoming jobs with shorter service times. However, two main challenges arise when applying size-based scheduling to LLM systems. First, accurately predicting output lengths from prompts is challenging and often resource-intensive, making it impractical for many systems. As a result, the state-of-the-art LLM systems default to first-come, first-served scheduling, which can lead to head-of-line blocking and reduced system efficiency. Second, preemption introduces extra memory overhead to LLM systems as they must maintain intermediate states for unfinished (preempted) requests. In this paper, we propose TRAIL, a method to obtain output predictions from the target LLM itself. After generating each output token, we recycle the embedding of its internal structure as input for a lightweight classifier that predicts the remaining length for each running request. Using these predictions, we propose a prediction-based SRPT variant with limited preemption designed to account for memory overhead in LLM systems. This variant allows preemption early in request execution when memory consumption is low but restricts preemption as requests approach completion to optimize resource utilization. On the theoretical side, we derive a closed-form formula for this SRPT variant in an M/G/1 queue model, which demonstrates its potential value. In our system, we implement this preemption policy alongside our embedding-based prediction method.

==> notes.tex <==


motivation
1) FCFS is ok when the job sizes are roughly the same
2) it is not the case in LLM (could be three orders of magnitude (explain different LLM tasks)

one could
migrate interference requests among decoding instances at
runtime based on predicted length


Metrics:
1) TTFT
2) JCT


when we have length predictions we cam implement:
non preemptable version
1) SJF - shortest job first
2) LJF - longest job first


preemptable version
2) SRPT
2) LRPT


deal with start-up


\section*{Modeling Refined Predictions as a Probability Function}

Given a job of size $X = x$, and a sequence of refined predictions $Y_0, Y_1, \dots, Y_x$, where $Y_i$ represents the prediction after processing $i$ units of $x$, we model the refined predictions as follows:

\subsection*{Conditional Probability}

The probability of the refined prediction $y_i$ at step $i$, given the actual size $x$ and the previous prediction $y_{i-1}$, is denoted as:
\[
P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1})
\]

\subsection*{Joint Probability Distribution}

The joint probability of the sequence of predictions $Y_0, Y_1, \dots, Y_x$ can be modeled as:
\[
P(Y_0 = y_0, Y_1 = y_1, \dots, Y_x = y_x \mid X = x) = P(Y_0 = y_0 \mid X = x) \prod_{i=1}^{x} P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1})
\]

\subsection*{Refining the Density Function}

The density function $g(x, y)$ corresponding to the final prediction after processing the entire job of size $x$ is obtained by summing over all possible refined predictions:
\[
g(x, y) = \sum_{y_0, y_1, \dots, y_{x-1}} P(Y_0 = y_0, Y_1 = y_1, \dots, Y_x = y \mid X = x)
\]

\subsection{Preemption with memory constraints}

Preemption in queueing theory reduces latency, but memory-constrained systems like Large Language Models (LLMs) present unique challenges. Jobs in LLMs consume memory upon scheduling and retain it until completion. In a fully utilized memory-constrained system, jobs cannot execute until memory is freed by other job completions. This scenario can lead to deadlock when no memory is available, preventing job completion and immediate scheduling of new jobs, even those with the shortest remaining processing time.
The Shortest Remaining Processing Time (SRPT) algorithm assumes immediate context switching for theoretical optimality. However, memory constraints violate this assumption by preventing immediate scheduling of shorter jobs due to insufficient memory.
To address these challenges, we propose SRPT with memory reservation. This approach reserves memory for each scheduled job, ensuring sufficient memory availability when shorter jobs need to preempt longer ones. Since memory and job size (input and output) correlate, memory reservation maintains SRPT principles.
The proposed method reserves memory for job j upon scheduling based on its input (i_j) and predicted output (y_j), or a linear function of these parameters. This reservation ensures memory availability for new, shorter jobs. When a shorter job arrives, the system preempts (pauses) the current job while maintaining its memory allocation. The new job is then scheduled, and upon completion, its memory is freed, allowing the paused job to resume.
This approach aims to mitigate the impact of memory constraints on SRPT performance in LLM systems.

\begin{itemize}
    \item 
    Preemption helps achieve lower latency according to queueing theory. Howeverm, in LLM which is a memory-constrained system, each job consumes memory upon scheduling and frees it only after completion.
    \item In a fully utilized memory-constrained system, a scheduled job cannot execute until memory is freed by another job's completion. However, when no memory is available, a deadlock arises - no job can complete to free memory, and no memory can be freed to run a job. In addition, a new job cannot be immediately scheduled, even if it has the shortest remaining processing time.
    \item 
    SRPT's theoretical optimality assumes an immediate context switch, but memory constraints violate this by preventing immediate scheduling of shortest remaining time jobs due to insufficient memory.
    \item 

    To mitigate the impact of memory constraints, the system could consider SRPT with memory reservation.
    This variant reserves memory for each scheduled job, ensuring that sufficient memory is available when a shorter job needs to preempt a longer one. Since memory and job size (input and output) are correlated, so reserving memory doesn't violate SPRT

    \item Reserve memory for job $j$ upon scheduling according to input ($i_j$) and output prediction $y_j$ (or some linear function of them), which ensures memory availability for new shorter jobs.

    \item If a shorter job arrives, preempt (pause) the current job and keep its memory allocated

    \item Schedule the new job, when it completes, its memory is freed, so we can resume the paused job.
\end{itemize}


\paragraph{Optimality of the scheduling algorithm}

\begin{theorem}
    With memory reservation, a shorter job can always be scheduled immediately upon arrival.
\end{theorem}

\begin{theorem}
    Memory reservation prevents deadlocks, ensuring all jobs eventually run to completion.
\end{theorem}

\begin{theorem}
    The modified SRPT with memory reservation minimizes the mean response time under memory constraints.
\end{theorem}




==> sections/theory.tex <==
\section{Theory}



\subsection{Limited Preemption}

We focus on limiting preemptions per job to address memory constraints. Early in the job's execution, preemptions are less costly since minimal resources have been consumed. However, as the job nears completion, avoiding preemption becomes critical to ensure timely completion. To manage this, we introduce a job descriptor \((x, r), a\), and define a threshold \(a_0 = C \cdot x\) (where \(C\) can be determined, when $C=1$ it is SPRPT). Before reaching \(a_0\), the rank function is \(r - a\), allowing preemption. Once \(a_0\) is exceeded, preemption is disabled by setting the rank function to \(-\infty\).


    
SPRPT with limited preemption has a rank function for job of size $x$ and predicted size $r$

\[
rank((x,r), a)  = 
\begin{cases} 
r-a & \text{if } a < a_0 \\
-\infty  & else
\end{cases}
\]
\rana{we can also use $-a$ instead of $-\infty$}

As this rank function is monotonic, $J$'s worst future rank is its initial prediction:

\[
rank_{d_J, x_J}^{\text{worst}} (a)  = 
\begin{cases} 
r-a_0 & \text{if } a < a_0 \\
-\infty  & else
\end{cases}
\]

When $a_J=0$, the rank function is denoted by $r_{worst}= rank_{d_J, x_J}^{\text{worst}} (0) = r$.



\begin{lemma}
\label{lem:sprpt_ext}
    For SPRPT with limited preemption, where at age $a_0$ the jobs become non-presentable, the expected mean response time for a job of true size $x_J$ and predicted size $r$ is
    
    \begin{align*}
\mathbb{E}[T(x_J, r)]^{{SPRPT}} = &\frac{\lambda \left(\int_{y = 0}^{r} \int_{x_I = 0}^{\infty} x_I^2\cdot  g(x_I, y) dx_I dy + \int_{t = r + a_0}^{\infty} \int_{x_I = t-r}^{\infty} g(x_I, t) \cdot(x_I - (t - r))^2 \cdot dx_I dt\right)}{2(1-\rho'_r)^2} \\
&+ \int_{0}^{a_0} \frac{1}{1-\rho'_{(r-a)^+}} \, da + (x_J - a_0).
\end{align*}
 where $\rho'_r= \lambda \int_{y = 0}^{r} \int_{x_I = 0}^{\infty} x_I \cdot g(x_I,y) dx_I dy$.
\end{lemma}

\begin{proof}
    
\subsubsection{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ computation:}
Suppose that a new job $K$ of predicted size $r_K$ arrives when $J$ has age $a$.
If $a < a_0$ and $K$ has a predicted job size less than $J$'s predicted remaining process time ($r - a$), $K$ will always outrank $J$. Thus



\[
X_{x_K}^{\text{new}}[r - a] = x_K \mathbf{1}(r_K < r - a) \mathbf{1}(a < a_0)
\]


\begin{align*}
\mathbb{E}[X^{new}[r - a]] = \int_{0}^{r-a} \int_{x_K = 0}^{\infty} x_K \cdot g(x_K,y) dx_K dy \\
\end{align*}


\subsubsection{$X_{0}^{\text{old}}[r_{worst}]$ computation:}
Whether job $I$ is an original or recycled job depends on its predicted size relative to J's predicted size.
If $r_I \le r$, then $I$ is original until its completion because its rank never exceeds $r$.

\[
X_{0, x_I}^{\text{old}}[r] = x_I\mathds{1}(r_I \le r).
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[r]] = \int_{y = 0}^{r} \int_{x_I = 0}^{\infty} x_I \cdot g(x_I,y) dx_I dy.
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[r])^2]] = \int_{y = 0}^{r} \int_{x_I = 0}^{\infty} x_I^2 \cdot g(x_I, y) dx_I dy.
\end{align*}







\subsubsection{$X_{i}^{\text{old}}[r_{worst}]$ computation:}
If $r_I > r$, then $I$ starts discarded but becomes recycled when $r_I - a = r$. This means at age $a = r_I -r$ and served till completion only if $a<a_0$, which will be $x_I - a_I = x_I - (r_I - r)$:

Thus, we have
\[
X_{1, x_I}^{\text{old}}[r] = x_I - (r_I- r).
\]
For $i \ge 2$, $$X_{i, x_I}^{\text{old}}[r] = 0.$$



\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[r]^2] = \int_{r_I= r + a_0}^{\infty} \int_{x_I = r_I-r}^{\infty} g(x_I, t) \cdot (x_I - (r_I- r))^2 \cdot dx_I dr_I.
\end{align*}



Applying Theorem 5.5 of SOAP~\citep{scully2018soap} yields that the mean response time of jobs with descriptor ($r$) and size $x_J$ is as follows.
Let
$$\rho'_r= \lambda \int_{y = 0}^{r} \int_{x_I = 0}^{\infty} x_I \cdot g(x_I,y) dx_I dy.$$
Then

\begin{align*}
\mathbb{E}[T(x_J, r)]^{{SPRPT}} = &\frac{\lambda \left(\int_{y = 0}^{r} \int_{x_I = 0}^{\infty} x_I^2\cdot  g(x_I, y) dx_I dy + \int_{t = r + a_0}^{\infty} \int_{x_I = t-r}^{\infty} g(x_I, t) \cdot(x_I - (t - r))^2 \cdot dx_I dt\right)}{2(1-\rho'_r)^2} \\
&+ \int_{0}^{a_0} \frac{1}{1-\rho'_{(r-a)^+}} \, da + (x_J - a_0).
\end{align*}

Let $f_p(y) = \int_{x=0}^{\infty} g(x,y) dx$. Then the mean response time for a job with size $x_J$, and the mean response time over all jobs are given by 
$$\mathbb{E}[T(x_J)] = \int_{y=0}^{\infty} f_p(y) \mathbb{E}[T(x_J,y)] dy,$$


$$\mathbb{E}[T]^{{SPRPT}} = \int_{x=0}^{\infty} \int_{y=0}^{\infty} g(x,y)  \mathbb{E}[T(x,y)] dy dx.$$



%\todo[inline]{Compare SPRPT with/without limited prediction as a function of C, when C=0, it should be SJF, and when C=1, it should be SPRPT without limitation. In the comparison, include the memory consumption, we should see with higher C (towards 1), when we have high memory consumption but good mean response time and with low C the opposite, we want to be in the middle.}
\end{proof}



\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figures/limited_P_sim/new_new_response_memory_vs_arrival_C_val_0.0.png}
        \caption{vs. arrival rate when $C=0$}
        \label{fig:fig1}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figures/limited_P_sim/new_new_response_memory_vs_arrival_C_val_0.8.png}
        \caption{vs. arrival rate when $C=0.8$}
        \label{fig:fig2}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figures/limited_P_sim/new_new_response_memory_vs_arrival_C_val_1.0.png}
        \caption{vs. arrival rate when $C=1$}
        \label{fig:fig3}
    \end{minipage}
    
    \vskip\baselineskip  % Add vertical space between rows
    
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figures/limited_P_sim/new_new_response_memory_vs_c_arrival_rate_0.8.png}
        \caption{vs. $C$ when $\lambda=0.8$}
        \label{fig:fig4}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figures/limited_P_sim/new_new_response_memory_vs_c_arrival_rate_0.9.png}
        \caption{vs. $C$ when $\lambda=0.9$}
        \label{fig:fig5}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figures/limited_P_sim/new_new_response_memory_vs_c_arrival_rate_0.95.png}
        \caption{vs. $C$ when $\lambda=0.95$}
        \label{fig:fig6}
    \end{minipage}
\end{figure}



Overall performance can be defined as the sum of the job's expected response time and the peak memory usage.


\subsection{Refined Predictions}

We consider M/G/1 queueing systems with arrival rate $\lambda$. The processing times for each arriving job are independent and drawn based on the cumulative distribution $F(x)$, with an associated density function $f(x)$.



Given a job of size $X = x$, and a sequence of refined predictions $Y_0, Y_1, \dots, Y_x$, where $Y_i$ represents the prediction after processing $i$ units of $x$, we model the refined predictions as follows:


The probability of the refined prediction $y_i$ at step $i$, given the actual size $x$ and the entire history of previous predictions, is denoted as:
\[
P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1}, Y_{i-2} = y_{i-2}, \dots, Y_0 = y_0)
\]


Under the Markovian assumption, the refined prediction at step $i$ depends only on the actual size $x$ and the previous prediction $y_{i-1}$:
\[
P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1}, Y_{i-2} = y_{i-2}, \dots, Y_0 = y_0) = P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1})
\]


The joint probability of the sequence of predictions $Y_0, Y_1, \dots, Y_x$ can be modeled as:
\[
P(Y_0 = y_0, Y_1 = y_1, \dots, Y_x = y_x \mid X = x) = P(Y_0 = y_0 \mid X = x) \prod_{i=1}^{x} P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1})
\]



The density function $g(x, y)$ corresponding to the list of predictions $y = [y_0, y_1, \dots, y_{x-1}]$, where each $y_i$ is obtained after processing one unit of job $x$, is obtained by summing over all possible refined predictions:
\[
g(x, y) = \sum_{y_0=0}^{\infty} \sum_{y_1=0}^{\infty} \dots \sum_{y_{x-1}=0}^{\infty} P(Y_0 = y_0, Y_1 = y_1, \dots, Y_{x-1} = y_{x-1} \mid X = x)
\]

\subsection{SPRPT with refined predictions}
The relevant attributes are size and the refined prediction list $r$.
We can model the system using descriptor $\mathcal{D} =$ [size, list of refined predictions] $= [x,r]$.
    
SPRPT has a rank function $rank(r, a) = r[a] - a$ for job of size $x$ and predicted size $r[a]$ at time $a$. We denote the maximum rank function as $r_{max}$.

$J$'s worst future rank is:
\[
rank_{d_J, x_J}^{\text{worst}}(a)= \sup_{a < b < x} (r[b] - b) = \max_{a < b < x} (r[b] - b)
\]


When $a_J=0$, the rank function is denoted by $r_{worst}= rank_{d_J, x_J}^{\text{worst}} (0) = r_{max}$.






\subsubsection{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ computation:}
Suppose that a new job $K$ of predicted size $r_K$ arrives when $J$ has age $a$. 


Let $ a_{J_0}$ be the age of job $ J$ when job $ K$ arrives. %The corresponding age of job $ K$ at each step $ i$ is $ a_K[i] = a_J[i] - a_{J_0}$.

$ K$ has a lower rank than the worst possible rank of job $ J$ is given by:






\[
X_{x_K}^{new}[rank_{d_J, x_J}^{\text{worst}}(a)]  = \sum_{a_K=0}^{x_K}  \mathbf{1}\left(r_K[a_K] - a_K < \max_{a_{J_0} < b < x_J} (r[b] - b)\right) \cdot \mathbf{1}\left(\forall j < a_I, \, r_I[j] - j < \max_{a_{J_0} < b < x_J} (r[b] - b)\right)
\]

where $ \mathbf{1}(\cdot)$ is the indicator function, which equals 1 if the condition inside is true and 0 otherwise.


\begin{align*}
\mathbb{E}[X^{new}[rank_{d_J, x_J}^{\text{worst}}(a)] ]= \sum_{x_K=0}^{\infty} \left( \sum_{a_K=0}^{x_K}  \mathbf{1}\left(r_K[a_K] - a_K < \max_{a_{J_0} < b < x_J} (r[b] - b)\right) \\  \cdot \mathbf{1}\left(\forall j < a_I, \, r_I[j] - j < \max_{a_{J_0} < b < x_J} (r[b] - b)\right) \right) \cdot g(x_K, y)
\end{align*}

where the density function $ g(x_K, y)$ is defined as:

\[
g(x_K, y) = \sum_{y_0=0}^{\infty} \sum_{y_1=0}^{\infty} \dots \sum_{y_{x_K-1}=0}^{\infty} P(Y_0 = y_0, Y_1 = y_1, \dots, Y_{x_K-1} = y_{x_K-1} \mid X = x_K)
\]



\subsubsection{$X_{0}^{\text{old}}[r_{worst}]$ computation:}
Whether job $I$ is an original depends on its predicted size relative to J's predicted size.
$I$ is original till it is exceeds $r_{max}$. we terminate the summing once you encounter an age where $r_I[a_I] - a_I > r_{max}$

\[
X_{0, x_I}^{\text{old}}[r_{max}] = \sum_{a_I=0}^{x_I} \mathbf{1}\left(r_I[a_I] - a_I < r_{max} \right) \cdot \mathbf{1}\left(\forall j < a_I, \, r_I[j] - j < r_{max}\right)
\]
%\[X_{0, x_I}^{\text{old}}[r_{max}] = \sum_{a_I=0}^{x_I}  \mathbf{1}\left(r_I[a_I] - a_I < r_{max}\right)\]



\subsubsection{$X_{i}^{\text{old}}[r_{worst}]$ computation:}
If $r_I > r$, then $I$ starts discarded but becomes recycled when $r_I[a] - a = r_{worst}$. This means at age $a = r_I[a_I] -r_{worst}$ and served till it will be again about $r_{worst}$,

\begin{comment}
Let interval $ m$ start at age $ a_{m, \text{start}}$ and end at age $ a_{m, \text{end}}$.

The summation for interval $ m$, where the rank of job $ I$ is less than $ r_{max}$, and before and after the interval, the rank is higher, is given by:

\[
X_{m}^{\text{OLD}}[r_{max}] = \sum_{a_I = a_{m,\text{start}}}^{a_{m,\text{end}}} \mathbf{1}\left(r_I[a_I] - a_I < r_{max} \right) \cdot \mathbf{1}\left(\forall j < a_{m,\text{start}}, \, r_I[j] - j > r_{max}\right) \cdot \mathbf{1}\left(\forall k > a_{m,\text{end}}, \, r_I[k] - k > r_{max}\right)
\]




%======== UNDERTSAND FORM PAPER AND CONTIBUE!!
which will be $x_I - a_I = x_I - (r_I - r)$,  let $t = r_I$:


\end{comment}




Let  $i$ be an interval index. The $i$-interval for job $ I$ is defined as the interval of ages during which the rank of job $ I$ is less than $ r_{max}$. Specifically:

\[
b_0[r] = 0
\]
This indicates that the first interval starts at age 0.

\[
c_0[r] = \inf \{a > 0 \mid r_I(a) - a > r_{max} \}
\]
Here, $ c_0[r]$ is the smallest age greater than 0 where the rank function $ r_I(a) - a$ becomes greater than $ r_{max}$, marking the end of the first interval where the rank is less than $ r_{max}$.

For subsequent intervals $i\geq 1$:

\[
b_i[r] = \inf \{a \geq c_{i-1}[r] \mid r_I(a) - a < r_{max} \}
\]
This is the starting point of the $i$-th interval, which begins as soon as the rank $ r_I(a) - a$ drops below $ r_{max}$ again after the previous interval $ [b_{i-1}[r], c_{i-1}[r]]$.

\[
c_i[r] = \inf \{a > b_i[r] \mid r_I(a) - a > r_{max} \}
\]
Here, $ c_i[r]$ is the endpoint of the $i$-th interval, where the rank $ r_I(a) - a$ becomes greater than $ r_{max}$ again.



For $i\geq 0$, the $i$-interval work is a random variable, written $ X_i^{\text{OLD}}[r]$, representing the sum of the tokens where job $ I$ has rank less than $ r_{max}$ within its $i$-interval.

\[
X_i^{\text{OLD}}[r] = 
\begin{cases} 
0 & \text{if } X_d < b_i[r] \\
X_d - b_i[r] & \text{if } b_i[r] \leq X_d < c_i[r] \\
c_i[r] - b_i[r] & \text{if } c_i[r] \leq X_d
\end{cases}
\]

If $ b_i[r] = c_i[r] = \infty$, we define $ X_i^{\text{OLD}}[r] = 0$.


\todo[inline]{prove with one refined prediction and then we can make it more general with any number of refined predictions}

\begin{comment}
    
Given a job of size $X = x$, and a sequence of refined predictions $Y_0, Y_1, \dots, Y_x$, where $Y_i$ represents the prediction after processing $i$ units of $x$, we model the refined predictions as follows:


The probability of the refined prediction $y_i$ at step $i$, given the actual size $x$ and the previous prediction $y_{i-1}$, is denoted as:
\[
P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1}, Y_{i-2} = y_{i-2}, \cdots)
\]

The joint probability of the sequence of predictions $Y_0, Y_1, \dots, Y_x$ can be modeled as:
\[
P(Y_0 = y_0, Y_1 = y_1, \dots, Y_x = y_x \mid X = x) = P(Y_0 = y_0 \mid X = x) \prod_{i=1}^{x} P(Y_i = y_i \mid X = x, Y_{i-1} = y_{i-1}, Y_{i-2} = y_{i-2}, \cdots)
\]

The density function $g(x, y)$ corresponding to the final prediction after processing the entire job of size $x$ is obtained by summing over all possible refined predictions:
\[
g(x, y) = \sum_{y_0, y_1, \dots, y_{x-1}} P(Y_0 = y_0, Y_1 = y_1, \dots, Y_x = y \mid X = x)
\]
\end{comment}

